Instruction Tuning for Few-Shot Aspect-Based Sentiment Analysis

Aspect-based Sentiment Analysis (ABSA) is a fine-grained sentiment analysis task which involves four elements from user-generated texts: aspect term, aspect category, opinion term, and sentiment polarity. Most computational approaches focus on some of the ABSA sub-tasks such as tuple (aspect term, sentiment polarity) or triplet (aspect term, opinion term, sentiment polarity) extraction using either pipeline or joint modeling approaches. Recently, generative approaches have been proposed to extract all four elements as (one or more) quadruplets from text as a single task. In this work, we take a step further and propose a unified framework for solving ABSA, and the associated sub-tasks to improve the performance in few-shot scenarios. To this end, we fine-tune a T5 model with instructional prompts in a multi-task learning fashion covering all the sub-tasks, as well as the entire quadruple prediction task. In experiments with multiple benchmark datasets, we show that the proposed multi-task prompting approach brings performance boost (by absolute 8.29 F1) in the few-shot learning setting.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> error_analysis.tex <==
\section{Error Analysis}
\label{sec:error_analysis}



==> ethics.tex <==
\section*{Ethics Statement}
Scientific work published at EMNLP 2022 must comply with the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL Ethics Policy}. We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).

==> related_work.tex <==
\section{Related Work}
\label{sec:rel_work}

ABSA has been explored with discriminative approaches such as classification and extraction extensively in literature \cite{liu-etal-2015-fine,ma-etal-2019-exploring,wang2017coupled,li-etal-2019-exploiting,zhao-etal-2020-spanmlt,cai-etal-2021-aspect}. Recently, generative models have been shown to be effective for ABSA tasks \cite{zhang-etal-2021-towards-generative,zhang-etal-2021-aspect-sentiment,yan-etal-2021-unified}. 

\newcite{zhang-etal-2021-towards-generative}
%\miguel{this should be newcite not citeauthor} 
% Kishaloy to Migeul: Thanks for this! Adjusted.
attempt to use seq-to-seq model to solve ABSA and they approach the task as generative structured prediction similar to \cite{tanl-2021}. Like ours, it exploits contextual information such as aspect category names (\textit{e.g., food quality, restaurant ambiance}), sentiment classes (\textit{e.g., positive, negative}) in natural language. However, they keep the input unchanged and attempt to learn the overall triplet %\ignore{\neha{which is the triplet you are referring to here? Not clear from this statement}} 
% Kishaloy to Neha: Have introduced the triplet task in introduction now.
(or quadruplet in \cite{zhang-etal-2021-aspect-sentiment}) task at once. On the other hand, we consider the factorized sub-tasks and learn to solve all the variants of the same overall problem in a multi-task learning fashion using instructional prompts.
% \ignore{\neha{I suppose sentiment classes(positive, negative etc) and sentiment terms defined in ABSA(good, great, bad) are different, correct?}}
% Kishaloy to Neha: Not sure I fully understand the question. But in general the three sentiment classes are positive, negative, neutral.
%\robert{Maybe add that we learn them using instructions?}\shuai{We should highlight our difference, which are Instruction Tuning, MTL, and few-shot (our model do great for few-shot) .}
% Kishaloy to Robert: Adjusted the text.

%\miguel{If you do want to have a related work section, I miss a whole section on instruction tuning, prompt tuning, sequence to sequence models, task embeddings, etc. I think it would be better to include those citations listed above in the intro and introduce these concepts in the rest of the paper.}
% Kishaloy to Miguel: Agreed. However, since we just use some of these techniques as building blocks, I kept the related works limited to only most relevant works on the ABSA domain the paper being a short one. We have some overview around instruction tuning in the introduction. We could consider expanding if we have more space in the end.

% \shuai{The closest work should be Zhang et al., 2021, which does the text2text generation in a similar setting like ours, and we mainly compare ours results with that work. I cannot see why Shu et al. is closest or similar to our work, and we are not doing NLI. Also, you're introducing a "closest" work that we don't compare our results with, which is dangerous. I have (tentatively) commented out the following paragraph. We can write a paragraph to compare with Zhang et al., 2021 if needed.}

% Response to Shuai from Kishaloy: I agree with you that the generative text-to-text paradigm is similar to Zhang et al. However, that is already done and we are not claiming our novelty there. We are claiming the instruction tuning part as our main contribution. Shu et al use some hypothesis which look very similar to our instructions (at least to me). We can avoid the direct comparison though since they are using additional NLI data to train the model and essentially do a brute force search.

%Perhaps, closest to our approach was taken by \citeauthor{shu-2022-zero-shot}, where they try to cast ABSA as a Natural Language Inference task. They use the input text as the premise, some in-context as the hypothesis, and classify the pair into \textit{entailment, contradiction, neutral} classes. However, unlike ours, the approach requires non-trivial pre-processing to form relevant hypotheses from all possible spans in the input text. 

==> scratchpad.tex <==
% \begin{table}[]
%     \begin{subtable}[c]{.5\textwidth}
%         \centering
%         \resizebox{1\textwidth}{!}{%
%             \begin{tabular}{|c|c|c|c|c|c|c|}
%             %\hline
%             %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
%             \hline
%              \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
%             \\
%             \hline
%             \multirow{4 }{*}{AE}  & \textsc{BartAbsa} & 47.07 &	57.71 & 59.56 & -- & --\\ \cline{2-7} 
%             & Text & \textbf{48.06} &	\underline{61.42} &	66.67 &	70.38 &	78.13\\
%             & IT & \underline{47.99} & 61.2 & \underline{67.41} & \underline{71.03} & \underline{78.26}\\
%             & IT-MTL & 47.77 & \textbf{63.14} & \textbf{69.06} & \textbf{73.98} & \textbf{79.49}\\
%             \hline
%             \multirow{4 }{*}{AESC}  & \textsc{BartAbsa} & 31.82 &	45.83 &	49.95 & -- & --\\ \cline{2-7} 
%             & Text & 39.93 & 53.5 & 56.88 & 63.85 & \underline{72.16}\\
%             & IT & \textbf{42.46} & \textbf{55.39} & \underline{58.27} & \underline{64.93} & 71.49\\
%             & IT-MTL & \underline{42.39} & \underline{53.62} & \textbf{58.82} & \textbf{65.03} & \textbf{72.22}\\
%             \hline
%             \multirow{4 }{*}{TASD} & \textsc{Para.} & 23.59 & 39.65 & 44.46 & 50.78 & 63.06\\ 
%             \cline{2-7} 
%             & Text & \underline{24.49} & \underline{39.91} & \underline{47.66} & 55.21 & 64.02\\
%             & IT & 23.97 & 38.93 & 46.61 & \textbf{55.46} & \textbf{64.55}\\
%             & IT-MTL & \textbf{28.37} & \textbf{40.13} & \textbf{48.29} & \underline{55.39} & \underline{64.36} \\ \hline
%             \multirow{4 }{*}{ASTE} & \textsc{Para.} & 19.96 & 26.49 & 30.95 & 33.68 & \textbf{53.01} \\ 
%             \cline{2-7} 
%             & Text & 18.8 & 31.74 & 36.57 & 42.02 & 51.33\\
%             & IT & \underline{22.8} & \underline{32.84} & \underline{37.31} & \underline{42.29} & 51.78\\
%             & IT-MTL & \textbf{23.22} & \textbf{35.84} & \textbf{38.22} & \textbf{44.36} & \underline{52.95}\\
%             \hline
%             \multirow{4 }{*}{ASQP} & \textsc{Para.} & 12.25 & 20.84 & 24.49 & 28.26 & \underline{46.93}\\ 
%             \cline{2-7} 
%             & Text & 12.75 & 24.01 & 29.36 & 34.9 & 46.92\\
%             & IT & \underline{13.72} & \underline{25.05} & \underline{29.86} & \underline{37.29} & 46.93\\
%             & IT-MTL & \textbf{15.97} & \textbf{26.84} & \textbf{31.96} & \textbf{38.37} & \textbf{47.34}\\
%             \hline
%             \end{tabular}
%         }
%         \caption{\textsc{Rest15}}
%         \label{tab:results_rest15}
%     \end{subtable}
%     \begin{subtable}[c]{.5\textwidth}
%     \centering
%     \resizebox{1\textwidth}{!}{%
%         \begin{tabular}{|c|c|c|c|c|c|c|}
%             %\hline
%             %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
%             \hline
%              \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
%             \\
%             \hline
%             \multirow{4 }{*}{AE}  & \textsc{BartAbsa} & 55.60 &	61.68 & 64.59 & 72.99 & 80.55\\ \cline{2-7} 
%             & Text & 62.16& 69.2& 72.80& \textbf{79.58} & 84.10\\
%             & IT & \underline{64.82} & \underline{70.16} & \underline{73.91} & 79.20& \underline{84.31}\\
%             & IT-MTL & \textbf{66.58} & \textbf{72.64} & \textbf{75.15} & \underline{79.39} & \textbf{84.88}\\
%             \hline
%             \multirow{4 }{*}{AESC}  & \textsc{BartAbsa} & 46.60 &	52.08 &	55.44 & 64.35 & 74.91\\ \cline{2-7} 
%             & Text & \underline{56.38}& 61.39& 64.72& 70.71& 78.70 \\
%             & IT & 55.94& \textbf{62.96} & \underline{65.86} & \underline{70.73} & \textbf{79.30} \\
%             & IT-MTL & \textbf{58.90} & \underline{62.36} & \textbf{66.57} & \textbf{71.53} & \underline{79.20}\\
%             \hline
%             \multirow{4 }{*}{TASD} & \textsc{Para.} & 30.99 & 42.20 & 50.61& 55.99 & 71.97\\ 
%             \cline{2-7} 
%             & Text & 35.3& \underline{44.03} & 51.81& 59.54& 71.56\\
%             & IT & \underline{38.11} & 43.16& \underline{53.15} & \underline{61.56} & \textbf{72.14}\\
%             & IT-MTL &\textbf{46.13}& \textbf{48.18} & \textbf{53.77} & \textbf{61.59} & \underline{72.10} \\ \hline
%             \multirow{4 }{*}{ASTE} & \textsc{Para.} & 28.89 & 33.68 & 36.95 & 43.00 & 62.65 \\ 
%             \cline{2-7} 
%             & Text & 29.53& 39.84& 43.31& 52.21& \underline{63.14}\\
%             & IT & \underline{34.64} & \textbf{42.11} & \underline{44.9} & \underline{52.63} & \textbf{63.93}\\
%             & IT-MTL & \textbf{37.9} & \underline{41.65} & \textbf{45.89} & \textbf{54.32}& 62.9\\
%             \hline
%             \multirow{4 }{*}{ASQP} & \textsc{Para.} & 17.74 & 24.46 & 29.99 & 37.11 &
%             \textbf{57.93}\\  
%             \cline{2-7} 
%             & Text & 22.38& 29.84& 35.9& 46.78& 57.68\\
%             & IT & \underline{25.08} & \underline{31.33} & \underline{38.41} & \underline{47.93} & 57.70\\
%             & IT-MTL & \textbf{29.19} & \textbf{33.8} & \textbf{39.07} & \textbf{48.64} & \underline{57.90} \\
%             \hline
%         \end{tabular}
%         }
%         \caption{\textsc{Rest16}}
%         \label{tab:results_rest16}
%     \end{subtable}
%     \begin{subtable}[c]{.5\textwidth}
%     \centering
%     \resizebox{1\textwidth}{!}{%
%         \begin{tabular}{|c|c|c|c|c|c|c|}
%             %\hline
%             %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
%             \hline
%              \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
%             \\
%             \hline
%             \multirow{3 }{*}{AE}  & \textsc{BartAbsa} & 34.36 &	45.76 &	-- & -- & --\\ \cline{2-7} 
%             & Text & \textbf{34.69} & \underline{45.52} & 52.09 & 63.27 & 79.49 \\
%             & IT & \underline{34.34} & \textbf{49.04} & \textbf{54.37} & \textbf{65.77} & \underline{79.82}\\
%             & IT-MTL & 31.54 & 43.74 & \underline{54.01} & \underline{65.30} & \textbf{80.35}\\ \hline
%             \multirow{3 }{*}{AESC}  & \textsc{BartAbsa} & 16.26 &	35.80 &	-- & -- & --\\ \cline{2-7} 
%             & Text & 21.68 & 32.40 & 38.62 & 51.45 & \textbf{70.37}\\
%             & IT & \underline{23.28} & \textbf{36.76} & \underline{43.98} & \underline{53.93} & \underline{70.04}\\
%             & IT-MTL & \textbf{25.01} & \underline{34.66} & \textbf{44.96} & \textbf{54.95} & 69.41\\ \hline
%             \multirow{4 }{*}{ASTE} & \textsc{Para.} & \textbf{14.33} & \underline{22.31} & 27.96 & 33.85 & \textbf{61.13}\\
%             \cline{2-7} 
%             & Text & 10.10 & 16.27 & 26.8 & 40.38 & 58.92\\
%             & IT & 12.60 & 21.35 & 30.38 & 42.96 & \underline{60.37}\\
%             & IT-MTL & \underline{14.18} & \textbf{24.09} & \textbf{32.89} & \textbf{43.62} & 59.15\\
%             \hline
%         \end{tabular}
%         }
%         \caption{\textsc{Laptop14}}
%         \label{tab:results_laptop14}
%     \end{subtable}
% %\vspace{-2mm}
% \caption{Results on (a) \textsc{Rest15}, (b) \textsc{Rest16}, (c) \textsc{Laptop14} datasets for few($k$)-shot learning, and full dataset. Best is \textbf{bolded}, second-best is \underline{underlined}. Our proposed MTL outperforms \textsc{Para}, and other ablations comfortably in most cases in few-shot scenarios.}
% \label{tab:all_task_results_dummy}
% \end{table}


\begin{table}[H]
    \begin{subtable}[c]{.5\textwidth}
        \centering
        \resizebox{1\textwidth}{!}{%
            \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{3 }{*}{AE}  & Text & 43.95 & 54.38 & 59.75 & 61.75 & 72.53\\
            & IT & \textbf{45.24} & 55.1 & 60.33 & 64.15 & 72.73\\
            & IT-MTL & 44.18 & \textbf{56.57} & \textbf{62.65} & \textbf{67.22} & \textbf{74.03}\\
            \hline
            \multirow{3 }{*}{AESC}  & Text & 37.33 & 47.68 & 50.6 & 56.69 & 66.2\\
            & IT & \textbf{39.4} & \textbf{49.43} & 52.06 & 58.4 & 66.49\\
            & IT-MTL & 38.99 & 47.62 & \textbf{53.58} & \textbf{59.54} & \textbf{67.06}\\
            \hline
            % \multirow{4 }{*}{TASD} & \textsc{Para.} & 22.13 & 33.74 & 39.44 & 45.16 & \textbf{60.07}\\
            \multirow{4 }{*}{TASD} & \textsc{Para.} & 21.34 & 37.39 & 42.52 & 47.57 & \textbf{60.00}\\
            \cline{2-7} 
            & Text & 22.55 & 36.37 & 42.28 & 48.52 & 58.93\\
            & IT & 22.92 & 36.52 & 43.2 & 50.14 & 59.46\\
            & IT-MTL & \textbf{27.05} & \textbf{36.81} & \textbf{43.56} & \textbf{50.24} & 59.76\\ \hline
            % \multirow{4 }{*}{ASTE} & \textsc{Para.} & 19.66 & 25.89 & 30.56 & 33.30 & \textbf{52.67} \\
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & 22.07 & 32.49 & 36.28 & 41.12 & \textbf{51.08} \\
            \cline{2-7} 
            & Text & 18.49 & 30.17 & 35.66 & 41.49 & 51.13\\
            & IT & 22.38 & 32.11 & 36.67 & 41.65 & 51.7\\
            & IT-MTL & \textbf{22.7} & \textbf{33.52} & \textbf{37.78} & \textbf{43.84} & 52.6\\
            \hline
            % \multirow{4 }{*}{ASQP} & \textsc{Para.} & 11.9 & 20.18 & 23.92 & 27.86 & 46.91\\
            \multirow{4 }{*}{ASQP} & \textsc{Para.} & 13.65 & 22.90 & 27.87 & 34.49 & 45.54\\
            \cline{2-7} 
            & Text & 12.15 & 22.19 & 28.82 & 33.96 & 46.79\\
            & IT & 13.3 & 24.35 & 29.66 & 36.78 & 46.59\\
            & IT-MTL & \textbf{15.54} & \textbf{25.46} & \textbf{31.47} & \textbf{37.72} & \textbf{46.99}\\
            \hline
            \end{tabular}
        }
        \caption{\textsc{Rest15}}
        \label{tab:results_rest15}
    \end{subtable}
    \begin{subtable}[c]{.5\textwidth}
    \centering
    \resizebox{1\textwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{3 }{*}{AE}  & Text & 52.7 & 58.5 & 61.49 & 67.21 & 78.57\\
            & IT & 55.64 & 59.36 & 63.75 & 68.14 & 79.09\\
            & IT-MTL & \textbf{59.41} & \textbf{61.87} & \textbf{66.88} & \textbf{71.18} & \textbf{79.41}\\
            \hline
            \multirow{3 }{*}{AESC}  & Text & 49.13 & 54.54 & 57.05 & 62.75 & 73.55\\
            & IT & 51.93 & 55.29 & 59.96 & 63.45 & \textbf{74.32}\\
            & IT-MTL & \textbf{52.42} & \textbf{55.37} & \textbf{60.22} & \textbf{65.14} & 74.07\\
            \hline
            % \multirow{4 }{*}{TASD} & \textsc{Para.} & 27.48 & 37.07 & 44.85 & 49.72 & \textbf{68.14}\\
            \multirow{4 }{*}{TASD} & \textsc{Para.} & 28.93 & 38.99 & 48.29 & 54.89 & \textbf{68.73}\\
            \cline{2-7} 
            & Text & 30.65 & 38.39 & 46.72 & 54.04 & 67.12\\
            & IT & 34.38 & 38.58 & 47.66 & 55.16 & 67.52\\
            & IT-MTL & \textbf{40.45} & \textbf{42.41} & \textbf{48.83} & \textbf{55.82} & 67.73\\ \hline
            % \multirow{4 }{*}{ASTE} & \textsc{Para.} & 27.84 & 32.39 & 36.18 & 41.72 & 62.09 \\
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & 32.48 & 38.90 & 43.51 & 51.47 & 62.02 \\
            \cline{2-7} 
            & Text & 28.44 & 38.23 & 42.12 & 50.9 & 62.68\\
            & IT & 33.08 & \textbf{41.12} & 44.08 & 51.69 & \textbf{63.49}\\
            & IT-MTL & \textbf{35.75} & 38.95 & \textbf{44.75} & \textbf{52.94} & 62.27\\
            \hline
            % \multirow{4 }{*}{ASQP} & \textsc{Para.} & 16.61 & 23.68 & 29.14 & 36.09 & \textbf{57.90}\\
            \multirow{4 }{*}{ASQP} & \textsc{Para.} & 20.02 & 28.58 & 36.26 & 43.50 & \textbf{57.37}\\
            \cline{2-7} 
            & Text & 20.98 & 28.06 & 35.04 & 45.26 &57.41 \\
            & IT & 23.86 & 30.02 & 37.2 & 46.9 & 57.48 \\
            & IT-MTL & \textbf{27.02} & \textbf{31.66} & \textbf{38.06} & \textbf{47.48} & 57.61 \\
            \hline
        \end{tabular}
        }
        \caption{\textsc{Rest16}}
        \label{tab:results_rest16}
    \end{subtable}
    \begin{subtable}[c]{.5\textwidth}
    \centering
    \resizebox{1\textwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{3 }{*}{AE}  & Text & \textbf{34.64} & 42.26 & 51.11 & 59.62 & 75.43\\
            & IT & 34.29 & \textbf{47.4} & 52.39 & \textbf{63.86} & 76.11\\
            & IT-MTL & 31.54 & 42.73 & \textbf{53.08} & 63.71 & \textbf{76.93}\\ \hline
            \multirow{3 }{*}{AESC}  & Text & 21.68 & 30.7 & 37.74 & 50.39 & \textbf{66.76}\\
            & IT & 23.28 & \textbf{36.55} & 43.39 & 52.92 & 65.97\\
            & IT-MTL & \textbf{25.01} & 34.44 & \textbf{44.5} & \textbf{53.75} & 66.07\\ \hline
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & \textbf{14.33} & \underline{22.00} & 27.71 & 33.40 & \textbf{60.70} \\
            \cline{2-7} 
            & Text & 10.1 & 16.27 & 26.37 & 39.65 & 58.69\\
            & IT & 12.6 & 21.31 & 30.03 & 41.91 & 60.14\\
            & IT-MTL & 14.18 & \textbf{24.09} & \textbf{32.39} & \textbf{42.62} & 58.74\\
            \hline
        \end{tabular}
        }
        \caption{\textsc{Laptop14}}
        \label{tab:results_laptop14}
    \end{subtable}
%\vspace{-2mm}
\caption{Results on (a) \textsc{Rest15}, (b) \textsc{Rest16}, (c) \textsc{Laptop14} datasets for few($k$)-shot learning, and full dataset with modified evaluation logic. Best is \textbf{bolded}, second-best is \underline{underlined}. Our proposed MTL outperforms \textsc{Para}, and other ablations comfortably in most cases in few-shot scenarios.}
\end{table}



\begin{table}[H]
    \begin{subtable}[c]{.5\textwidth}
        \centering
        \resizebox{1\textwidth}{!}{%
            \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{4 }{*}{AE}  & ABSABART & 19.68 &	42.99 &	57.43 &	63.48 &	77.12\\
            \cline{2-7}
            & Text & \textbf{48.06} &	\underline{61.42} &	66.67 &	70.38 &	78.13\\
            & IT & \underline{47.99} & 61.2 & \underline{67.41} & \underline{71.03} & \underline{78.26}\\
            & IT-MTL & 47.77 & \textbf{63.14} & \textbf{69.06} & \textbf{73.98} & \textbf{79.49}\\
            \hline
            \multirow{3 }{*}{AESC} & ABSABART & 10.77 &	27.38 &	42.23 &	52.55 &	67.85\\
            \cline{2-7}
            & Text & 39.93 & 53.5 & 56.88 & 63.85 & \underline{72.16}\\
            & IT & \textbf{42.46} & \textbf{55.39} & \underline{58.27} & \underline{64.93} & 71.49\\
            & IT-MTL & \underline{42.39} & \underline{53.62} & \textbf{58.82} & \textbf{65.03} & \textbf{72.22}\\
            \hline
            \multirow{4 }{*}{TASD} & \textsc{Para.} & 23.59 & 39.65 & 44.46 & 50.78 & 63.06\\ 
            \cline{2-7} 
            & Text & \underline{24.49} & \underline{39.91} & \underline{47.66} & 55.21 & 64.02\\
            & IT & 23.97 & 38.93 & 46.61 & \textbf{55.46} & \textbf{64.55}\\
            & IT-MTL & \textbf{28.37} & \textbf{40.13} & \textbf{48.29} & \underline{55.39} & \underline{64.36} \\ \hline
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & 19.96 & 26.49 & 30.95 & 33.68 & \textbf{53.01} \\ 
            \cline{2-7} 
            & Text & 18.8 & 31.74 & 36.57 & 42.02 & 51.33\\
            & IT & \underline{22.8} & \underline{32.84} & \underline{37.31} & \underline{42.29} & 51.78\\
            & IT-MTL & \textbf{23.22} & \textbf{35.84} & \textbf{38.22} & \textbf{44.36} & \underline{52.95}\\
            \hline
            \multirow{4 }{*}{ASQP} & \textsc{Para.} & 12.25 & 20.84 & 24.49 & 28.26 & \underline{46.93}\\ 
            \cline{2-7} 
            & Text & 12.75 & 24.01 & 29.36 & 34.9 & 46.92\\
            & IT & \underline{13.72} & \underline{25.05} & \underline{29.86} & \underline{37.29} & 46.93\\
            & IT-MTL & \textbf{15.97} & \textbf{26.84} & \textbf{31.96} & \textbf{38.37} & \textbf{47.34}\\
            \hline
            \end{tabular}
        }
        \caption{\textsc{Rest15}}
        \label{tab:results_rest15}
    \end{subtable}
    \begin{subtable}[c]{.5\textwidth}
    \centering
    \resizebox{1\textwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{4}{*}{AE} & ABSABART & 31.48 & 55.90 & 62.96 & 71.06 & 80.95\\
            \cline{2-7}
            & Text & 62.16& 69.2& 72.80& \textbf{79.58} & 84.10\\
            & IT & \underline{64.82} & \underline{70.16} & \underline{73.91} & 79.20& \underline{84.31}\\
            & IT-MTL & \textbf{66.58} & \textbf{72.64} & \textbf{75.15} & \underline{79.39} & \textbf{84.88}\\
            \hline
            \multirow{4 }{*}{AESC} & ABSABART & 25.45 & 46.31 & 53.27 & 62.90 & 74.37\\
            \cline{2-7}
            & Text & \underline{56.38}& 61.39& 64.72& 70.71& 78.70 \\
            & IT & 55.94& \textbf{62.96} & \underline{65.86} & \underline{70.73} & \textbf{79.30} \\
            & IT-MTL & \textbf{58.90} & \underline{62.36} & \textbf{66.57} & \textbf{71.53} & \underline{79.20}\\
            \hline
            \multirow{4 }{*}{TASD} & \textsc{Para.} & 30.99 & 42.20 & 50.61& 55.99 & 71.97\\ 
            \cline{2-7} 
            & Text & 35.3& \underline{44.03} & 51.81& 59.54& 71.56\\
            & IT & \underline{38.11} & 43.16& \underline{53.15} & \underline{61.56} & \textbf{72.14}\\
            & IT-MTL &\textbf{46.13}& \textbf{48.18} & \textbf{53.77} & \textbf{61.59} & \underline{72.10} \\ \hline
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & 28.89 & 33.68 & 36.95 & 43.00 & 62.65 \\ 
            \cline{2-7} 
            & Text & 29.53& 39.84& 43.31& 52.21& \underline{63.14}\\
            & IT & \underline{34.64} & \textbf{42.11} & \underline{44.9} & \underline{52.63} & \textbf{63.93}\\
            & IT-MTL & \textbf{37.9} & \underline{41.65} & \textbf{45.89} & \textbf{54.32}& 62.9\\
            \hline
            \multirow{4 }{*}{ASQP} & \textsc{Para.} & 17.74 & 24.46 & 29.99 & 37.11 &
            \textbf{57.93}\\  
            \cline{2-7} 
            & Text & 22.38& 29.84& 35.9& 46.78& 57.68\\
            & IT & \underline{25.08} & \underline{31.33} & \underline{38.41} & \underline{47.93} & 57.70\\
            & IT-MTL & \textbf{29.19} & \textbf{33.8} & \textbf{39.07} & \textbf{48.64} & \underline{57.90} \\
            \hline
        \end{tabular}
        }
        \caption{\textsc{Rest16}}
        \label{tab:results_rest16}
    \end{subtable}
    \begin{subtable}[c]{.5\textwidth}
    \centering
    \resizebox{1\textwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{4}{*}{AE} & ABSABART & -- & 5.54 & 33.04 & 60.98 & \textbf{82.84}\\
            \cline{2-7}
            & Text & \textbf{34.69} & \underline{45.52} & 52.09 & 63.27 & 79.49 \\
            & IT & \underline{34.34} & \textbf{49.04} & \textbf{54.37} & \textbf{65.77} & 79.82\\
            & IT-MTL & 31.54 & 43.74 & \underline{54.01} & \underline{65.30} & \underline{80.35}\\ \hline
            \multirow{4}{*}{AESC} & ABSABART & -- & 4.75 & 24.92 & 50.01 & 69.54\\
            \cline{2-7}
            & Text & 21.68 & 32.40 & 38.62 & 51.45 & \textbf{70.37}\\
            & IT & \underline{23.28} & \textbf{36.76} & \underline{43.98} & \underline{53.93} & \underline{70.04}\\
            & IT-MTL & \textbf{25.01} & \underline{34.66} & \textbf{44.96} & \textbf{54.95} & 69.41\\ \hline
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & \textbf{14.33} & \underline{22.31} & 27.96 & 33.85 & \textbf{61.13}\\
            \cline{2-7} 
            & Text & 10.10 & 16.27 & 26.8 & 40.38 & 58.92\\
            & IT & 12.60 & 21.35 & 30.38 & 42.96 & \underline{60.37}\\
            & IT-MTL & \underline{14.18} & \textbf{24.09} & \textbf{32.89} & \textbf{43.62} & 59.15\\
            \hline
        \end{tabular}
        }
        \caption{\textsc{Laptop14}}
        \label{tab:results_laptop14}
    \end{subtable}
%\vspace{-2mm}
\caption{[ABSABART W/ OLD EVALUATION NUMBERS] Results on (a) \textsc{Rest15}, (b) \textsc{Rest16}, (c) \textsc{Laptop14} datasets for few($k$)-shot learning, and full dataset. Best is \textbf{bolded}, second-best is \underline{underlined}. Our proposed MTL outperforms \textsc{Para}, and other ablations comfortably in most cases in few-shot scenarios.}
\label{tab:all_task_results}
\end{table}

\begin{table}[H]
    \begin{subtable}[c]{.5\textwidth}
        \centering
        \resizebox{1\textwidth}{!}{%
            \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{4 }{*}{AE}  & BARTABSA & 19.68 &	42.99 &	57.43 &	63.48 &	77.12\\
            \cline{2-7}
            & Text & 43.95 & 54.38 & 59.75 & 61.75 & 72.53\\
            & IT & \textbf{45.24} & 55.1 & 60.33 & 64.15 & 72.73\\
            & IT-MTL & 44.18 & \textbf{56.57} & \textbf{62.65} & \textbf{67.22} & \textbf{74.03}\\
            \hline
            \multirow{4 }{*}{AESC} & BARTABSA & 10.77 &	27.38 &	42.23 &	52.55 &	67.85\\
            \cline{2-7}
            & Text & 37.33 & 47.68 & 50.6 & 56.69 & 66.2\\
            & IT & \textbf{39.4} & \textbf{49.43} & 52.06 & 58.4 & 66.49\\
            & IT-MTL & 38.99 & 47.62 & \textbf{53.58} & \textbf{59.54} & \textbf{67.06}\\
            \hline
            % \multirow{4 }{*}{TASD} & \textsc{Para.} & 22.13 & 33.74 & 39.44 & 45.16 & \textbf{60.07}\\
            \multirow{4 }{*}{TASD} & \textsc{Para.} & 21.34 & 37.39 & 42.52 & 47.57 & \textbf{60.00}\\
            \cline{2-7} 
            & Text & 22.55 & 36.37 & 42.28 & 48.52 & 58.93\\
            & IT & 22.92 & 36.52 & 43.2 & 50.14 & 59.46\\
            & IT-MTL & \textbf{27.05} & \textbf{36.81} & \textbf{43.56} & \textbf{50.24} & 59.76\\ \hline
            % \multirow{4 }{*}{ASTE} & \textsc{Para.} & 19.66 & 25.89 & 30.56 & 33.30 & \textbf{52.67} \\
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & 22.07 & 32.49 & 36.28 & 41.12 & \textbf{51.08} \\
            \cline{2-7} 
            & Text & 18.49 & 30.17 & 35.66 & 41.49 & 51.13\\
            & IT & 22.38 & 32.11 & 36.67 & 41.65 & 51.7\\
            & IT-MTL & \textbf{22.7} & \textbf{33.52} & \textbf{37.78} & \textbf{43.84} & 52.6\\
            \hline
            % \multirow{4 }{*}{ASQP} & \textsc{Para.} & 11.9 & 20.18 & 23.92 & 27.86 & 46.91\\
            \multirow{4 }{*}{ASQP} & \textsc{Para.} & 13.65 & 22.90 & 27.87 & 34.49 & 45.54\\
            \cline{2-7} 
            & Text & 12.15 & 22.19 & 28.82 & 33.96 & 46.79\\
            & IT & 13.3 & 24.35 & 29.66 & 36.78 & 46.59\\
            & IT-MTL & \textbf{15.54} & \textbf{25.46} & \textbf{31.47} & \textbf{37.72} & \textbf{46.99}\\
            \hline
            \end{tabular}
        }
        \caption{\textsc{Rest15}}
        \label{tab:results_rest15}
    \end{subtable}
    \begin{subtable}[c]{.5\textwidth}
    \centering
    \resizebox{1\textwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{4}{*}{AE} & BARTABSA & 31.48 & 55.90 & 62.96 & 71.06 & 80.95\\
            \cline{2-7}  & Text & 52.7 & 58.5 & 61.49 & 67.21 & 78.57\\
            & IT & 55.64 & 59.36 & 63.75 & 68.14 & 79.09\\
            & IT-MTL & \textbf{59.41} & \textbf{61.87} & \textbf{66.88} & \textbf{71.18} & \textbf{79.41}\\
            \hline
            \multirow{4 }{*}{AESC} & BARTABSA & 25.45 & 46.31 & 53.27 & 62.90 & 74.37\\
            \cline{2-7}
            & Text & 49.13 & 54.54 & 57.05 & 62.75 & 73.55\\
            & IT & 51.93 & 55.29 & 59.96 & 63.45 & \textbf{74.32}\\
            & IT-MTL & \textbf{52.42} & \textbf{55.37} & \textbf{60.22} & \textbf{65.14} & 74.07\\
            \hline
            % \multirow{4 }{*}{TASD} & \textsc{Para.} & 27.48 & 37.07 & 44.85 & 49.72 & \textbf{68.14}\\
            \multirow{4 }{*}{TASD} & \textsc{Para.} & 28.93 & 38.99 & 48.29 & 54.89 & \textbf{68.73}\\
            \cline{2-7} 
            & Text & 30.65 & 38.39 & 46.72 & 54.04 & 67.12\\
            & IT & 34.38 & 38.58 & 47.66 & 55.16 & 67.52\\
            & IT-MTL & \textbf{40.45} & \textbf{42.41} & \textbf{48.83} & \textbf{55.82} & 67.73\\ \hline
            % \multirow{4 }{*}{ASTE} & \textsc{Para.} & 27.84 & 32.39 & 36.18 & 41.72 & 62.09 \\
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & 32.48 & 38.90 & 43.51 & 51.47 & 62.02 \\
            \cline{2-7} 
            & Text & 28.44 & 38.23 & 42.12 & 50.9 & 62.68\\
            & IT & 33.08 & \textbf{41.12} & 44.08 & 51.69 & \textbf{63.49}\\
            & IT-MTL & \textbf{35.75} & 38.95 & \textbf{44.75} & \textbf{52.94} & 62.27\\
            \hline
            % \multirow{4 }{*}{ASQP} & \textsc{Para.} & 16.61 & 23.68 & 29.14 & 36.09 & \textbf{57.90}\\
            \multirow{4 }{*}{ASQP} & \textsc{Para.} & 20.02 & 28.58 & 36.26 & 43.50 & \textbf{57.37}\\
            \cline{2-7} 
            & Text & 20.98 & 28.06 & 35.04 & 45.26 &57.41 \\
            & IT & 23.86 & 30.02 & 37.2 & 46.9 & 57.48 \\
            & IT-MTL & \textbf{27.02} & \textbf{31.66} & \textbf{38.06} & \textbf{47.48} & 57.61 \\
            \hline
        \end{tabular}
        }
        \caption{\textsc{Rest16}}
        \label{tab:results_rest16}
    \end{subtable}
    \begin{subtable}[c]{.5\textwidth}
    \centering
    \resizebox{1\textwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|c|c|}
            %\hline
            %\multicolumn{7}{|c|}{\rule{0pt}{8pt} \textbf{K Shot (or Full)}}   \\
            \hline
             \textbf{Task} &  \textbf{Model}   & \textbf{K=5}  & \textbf{K=10}  & \textbf{K=20} & \textbf{K=50} & \textbf{Full} 
            \\
            \hline
            \multirow{4}{*}{AE} & BARTABSA & -- & 5.54 & 33.04 & 60.98 & \textbf{82.84}\\
            \cline{2-7}
            & Text & \textbf{34.64} & 42.26 & 51.11 & 59.62 & 75.43\\
            & IT & 34.29 & \textbf{47.4} & 52.39 & \textbf{63.86} & 76.11\\
            & IT-MTL & 31.54 & 42.73 & \textbf{53.08} & 63.71 & \textbf{76.93}\\ \hline
            \multirow{4}{*}{AESC} & BARTABSA & -- & 4.75 & 24.92 & 50.01 & 69.54\\
            \cline{2-7}
            & Text & 21.68 & 30.7 & 37.74 & 50.39 & \textbf{66.76}\\
            & IT & 23.28 & \textbf{36.55} & 43.39 & 52.92 & 65.97\\
            & IT-MTL & \textbf{25.01} & 34.44 & \textbf{44.5} & \textbf{53.75} & 66.07\\ \hline
            \multirow{4 }{*}{ASTE} & \textsc{Para.} & \textbf{14.33} & \underline{22.00} & 27.71 & 33.40 & \textbf{60.70} \\
            \cline{2-7} 
            & Text & 10.1 & 16.27 & 26.37 & 39.65 & 58.69\\
            & IT & 12.6 & 21.31 & 30.03 & 41.91 & 60.14\\
            & IT-MTL & 14.18 & \textbf{24.09} & \textbf{32.39} & \textbf{42.62} & 58.74\\
            \hline
        \end{tabular}
        }
        \caption{\textsc{Laptop14}}
        \label{tab:results_laptop14}
    \end{subtable}
%\vspace{-2mm}
\caption{[ABSABART W/ NEW EVALUATION NUMBERS]  Results on (a) \textsc{Rest15}, (b) \textsc{Rest16}, (c) \textsc{Laptop14} datasets for few($k$)-shot learning, and full dataset with modified evaluation logic. Best is \textbf{bolded}, second-best is \underline{underlined}. Our proposed MTL outperforms \textsc{Para}, and other ablations comfortably in most cases in few-shot scenarios.}
\end{table}
